A Software-Defined QoS Provisioning Framework for HPC Applications

With the emergence of large-scale data-intensive high-performance applications, new I/O challenges appear in the efficient management of petabytes of information in High-Performance Computing (HPC) environments. Data management environments must meet the performance needs of such applications, represented by various Quality-of-Service (QoS) metrics such as desired bandwidth, response time guarantee, and resource utilization. Traditional high-performance management platforms are facing considerable challenges regarding flexibility, as well as the need to address a variety of QoS metrics and constraints. To tackle these challenges, a Software-Defined approach is considered promising, and various prototypes have already been deployed in Cloud-based data centers. In this paper, we investigate the idea of utilizing a software-defined approach to provide I/O QoS provisioning for HPC applications. We identify the key challenges towards the high degree of concurrency and variation in HPC platforms, and propose a series of novel designs into the general software-defined approach in order to deliver our goal. Specifically, we introduced a borrowing-based strategy and a new M-LWDF algorithm based on traditional token-bucket algorithms to assure a fair and efficient utilization of resources for HPC applications. Due to the lack of software-defined frameworks in current HPC platform, we evaluated our framework through simulation. The experimental results show that our strategies make a significant improvement upon the general HPC frameworks and lead to clear performance gain for HPC applications.

==> 11-Challenges.tex <==
\section{Challenges}
Even though the presented platform provides flexible mechanisms and traffic shaping capabilities to meet the QoS requirements, it still has two major challenges, and this study attempts to address them.
%
\begin{figure}[htbp]
	\begin{center}
		{\includegraphics[width=2.3in]{2.pdf}}
		\caption{Unbalanced IO requests.}
		\label{fig2}
	\end{center}
	\vspace{-1em}
\end{figure}
%

\subsubsection{\textbf{Unbalanced IO requests}}
HPC applications often perform IOs in an unbalanced way, which can cause a challenge for the fair sharing of tokens among storage servers. For example, Fig.~\ref{fig2} shows how this could happen. For simplicity, we only take one application as example. It issues unbalanced IO requests from different compute nodes hitting different storage servers. Suppose this application requests 300 MB/s bandwidth QoS, the total physical bandwidth limit for each storage is 500 MB/s, and the control plane assigns 300 MB/s tokens for this application. These tokens are evenly distributed to storage servers such that each of them has 100 MB/S tokens.
As this application only contains 100 MB/s tokens in each storage, server 1 could not serve requests at 150 MB/s, even though other servers actually have unused tokens for this application. In this example, only a total 250 MB/s bandwidth is provided even there are unused tokens for this application. To address such an issue, we propose a borrowing model described in the next section.

\subsubsection{\textbf{Physical limitation}}
Each storage server has a physical bandwidth limitation. This limitation can be reached due to unbalanced IO requests from a single application or due to the concurrent data accesses from multiple applications. If there is a need exceeding the limitation, even though there are tokens available, QoS requirement can not be satisfied. When this happens, the desired QoS of those applications should degraded. The degradation should be fair among multiple applications. 



==> 3.Motivation.tex <==
\section{Background}
\label{sec:3.Motivation}
\subsection{High Performance Computing Architecture}

\subsection{How I/O was done in HPC}

\subsection{Challenges}
\subsection{Software-Defined Approach}
Even though the presented platform provides flexible mechanisms and traffic shaping capabilities to meet the QoS requirements, it still has two major challenges, and this study attempts to address them.
%
\begin{figure}[htbp]
	\begin{center}
		{\includegraphics[width=2.3in]{2.pdf}}
		\caption{Unbalanced IO requests.}
		\label{fig2}
	\end{center}
	\vspace{-1em}
\end{figure}
%

\subsubsection{\textbf{Unbalanced IO requests}}
HPC applications often perform IOs in an unbalanced way, which can cause a challenge for the fair sharing of tokens among storage servers. For example, Fig.~\ref{fig2} shows how this could happen. For simplicity, we only take one application as example. It issues unbalanced IO requests from different compute nodes hitting different storage servers. Suppose this application requests 300 MB/s bandwidth QoS, the total physical bandwidth limit for each storage is 500 MB/s, and the control plane assigns 300 MB/s tokens for this application. These tokens are evenly distributed to storage servers such that each of them has 100 MB/S tokens.
As this application only contains 100 MB/s tokens in each storage, server 1 could not serve requests at 150 MB/s, even though other servers actually have unused tokens for this application. In this example, only a total 250 MB/s bandwidth is provided even there are unused tokens for this application. To address such an issue, we propose a borrowing model described in the next section.

\subsubsection{\textbf{Physical limitation}}
Each storage server has a physical bandwidth limitation. This limitation can be reached due to unbalanced IO requests from a single application or due to the concurrent data accesses from multiple applications. If there is a need exceeding the limitation, even though there are tokens available, QoS requirement can not be satisfied. When this happens, the desired QoS of those applications should degraded. The degradation should be fair among multiple applications. 








\subsection{Modified Largest Weighted Delay First (M- LWDF) Scheduler}

Modified Largest Weighted Delay First (M- LWDF) is an throughput-optimal scheduling algorithm that can be used to provide different forms of QoS (these forms of the QoS  were discussed in the Section~\ref{sec:2.Introduction}.
The MLWDF is used when a single shared resource (i.e., a single wireless link) is used for N users. Suppose we have N users in the system, and each of which has a queue of requests (i.e., packets or traffic) that need to be served
%suppose a queue is used for each user. Each queue receives a stream of data, and there is no way to control input rate.
We call a scheduling algorithm throughput-optimal if it is  able to handle all the predefined traffic without queues "blowing up" which means to keep all of them "stable". 

%For my information: Bandwidth is the raw capability of a communications channel to move data through that channel. Typically measured in bits or bytes per second (or some, possibly large, multiple thereof). May also be measured in hertz. Throughput is the total capability of a processing system to move product through that system. It can be measured in any quantifiable unit and may be measured in units relevant to the business process that the system supports (e.g. transactions or documents) rather than in technical units. 

\subsubsection{M- LWDF in the Network Theory}
In each time slot $t$, a queue $i$ will be served if the following value is maximal.
%
\begin{equation}
\gamma_i W_{i}(t)C_{i}(t)
\label{MLWDF}
\end{equation}
%
where $W_{i}(t)$ is the head-of-the-line (HOL)  packet delay for queue $i$, $C_{i}(t)$ is the channel capacity with respect to flow $i$ which change asynchronously in time~\cite{andrews2000cdma}, and $ \gamma_i$ are arbitrary positive constants. The HOL  packet delay refers to the delay of the first packet in a line of packets. 
The simulations reported in~\cite{andrews2000cdma} show that  M-LWDF scheduling algorithm performs very well when:
%
\begin{equation}
\gamma_i = \frac{a_{i}}{r_i}, \\
a_i = -\frac{\log{\delta_i}}{T_i}
\end{equation}
%
where ${r_i}$ is the average channel rate with respect to user i, $T_i $ is the desired delay thresholds ,$\delta_i$ is the desired maximum violation probability. In fact, parameter $a_i$ provides the QoS differentiation between the users and embodies the QoS requirements.  

Therefore the equation~\ref{MLWDF} can be written as follows:
%
\begin{equation}
-\frac{\log{\delta_i}}{T_i r_i} W_{i}(t)C_{i}(t)
\label{MLWDF2}
\end{equation}
%
So the channel capacity depends on the bandwidth (i.e., data transfer rate, which means the amount of data that can be transfered from one point to the another one in a given time period), and the channel capacity with respect to the user $i$ is equal to $C_{i}=\frac{availableRate_i}{averageRate}$, therefore for the user $i$ the equation~\ref{MLWDF2} can be written by:
%For my inforamation: in computer networks, bandwidth is used as a synonym for data transfer rate, the amount of data that can be carried from one point to another in a given time period (usually a second). Network bandwidth is usually expressed in bits per second (bps); 
%
\begin{equation}
-\frac{\log{(Prob(MaxViolation_i))}}{targetDelay_i}*
HOL_i*\frac{availableRate_i}{averageRate}
\end{equation}
%
Moreover, if for all users the delay $W_j(t)$ is replaced by the queue length (amount of data), the M-LWDF scheduling algorithm remains throughput-optimal~\cite{andrews2001providing}.% Both current channel conditions and the states of the queues play role in the scheduling decision.  which is the key feature of this algorithm. 

==> 5.SDN.tex <==
\section{Software-defined Network}
\label{sec:5.SDN}
Software-Defined Networking (SDN)~\cite{paruchuri2015future} is an emerging networking paradigm to deal with the limitations of the networks infrastructures.



==> 6.SDS.tex <==
\section{Proposed Software-Defined Storage Framework}
\label{sec:6.SDS}
Fig.~\ref{fig1} illustrates our proposed software-defined storage framework comprises three major layers; application layer, control layer, and storage layer. The first layer, the application layer, is formed of compute nodes running parallel applications such that I/O requirements per application are collected in queues inside the compute nodes. The second layer, the control layer which is the main contribution of this paper, used to monitor and control the entire framework. Actually, the control layer introduces a new layer in the I/O software stack which interposes a software above the file system layer but below the rest of the I/O software stack. Finally, the storage layer is used to manage the entire storage system. The storage layer directly talk to the control layer using a communication interface to program the data plane located inside the storages. The rest of this section explains each layer in detail.
%
\begin{figure}[htbp]
	\begin{center}
		{\includegraphics[width=3.6in]{1.pdf}}
		%\caption{QoS-Aware architecture using software-defined approach.}
		\caption{A software-defined QoS provisioning architecture for HPC applications}
		\label{fig1}
	\end{center}
\end{figure}
%
\subsection{Application layer}
This layer comprises compute nodes running HPC applications in a parallel fashion. Processes of the applications are distributed among compute nodes and most of their processing time devoted to I/O operations. As shown in Fig.~\ref{fig1}, the I/O requests are stored on dedicated queues of the compute nodes (i.e., one queue is assigned per compute node). These I/O requests (i.e., read or write) then must be moved to the storage layer to be executed. To this end, a communication interface between the application layer and the control layer used to send the dedicated compute node queues to the control layer. Then, these queues are classified to separate queues per application. Finally, the communication layer between the control layer and the storage layer is used to move the I/O requests to proper storages. 

\subsection{Control layer}
This layer consists of three major components; distributed data planes, centralized control plane, and  communication interfaces defined between the layers.  

\paragraph{Distributed data planes}
Distributed data planes comprises two level data planes. As shown in Fig.~\ref{fig1}, the first layer data plane, located on the control layer of the I/O software stack, called the global data plane consisting of only one data plane. However, the second layer data plane, called the local data plane, has a pool of local data planes located on the storage layer and distributed among entire storage servers. In general, data planes, no matter of being global or local, has the same architecture comprising three components; I/O classification, QoS specification, and M- LWDF scheduler. Each component is defined as follows: First, the \emph{I/O classification} component consists of a queue per application to classify the applications I/Os based on their I/O header. Because of this classification, I/O requests of the same application are put to the dedicated queue for that application. Another component is \emph{QoS (BW) specification} which collects desired QoS (bandwidth) requirement per application. Data plane also consists of MLWDF scheduler, which was explained in Section~\ref{sec:3.Background and Challenges}, to satisfy each individual QoS (bandwidth) requirements on a single shared storage server. In the following, the roles of two level data planes are explained in detail. Then different components of the data plane is discussed. 
%
\begin{enumerate}
	\item The global data plane collects I/O requests from the entire applications. These I/Os then classified to dedicated queues assigned per application. Classification is done based on the I/O headers such that requests with the same header belong to the same application and will be put to the same queue.
	%
	\item As shown in Fig.~\ref{fig1}, the pool of local data planes located on the storage layer (i.e., one local data plane for one storage server). Local data plane has the same functionality as the global one. However, the main difference between them is that the global data plane deal with the entire applications I/O requests in contrast, the local one only handles I/O requests issued on it.
\end{enumerate}
%

\paragraph{Centralized control plane}
\label{controlP}
It is a logically centralized component, called a controller, dictates the overall storage behaviour. It is the "brain" of the framework where control logic is implemented. This paradigm brings several benefits compared to traditional methods. First, it is much easier to introduce new storage behaviour in the storage servers through a software program. Second, it introduces the benefits of a centralized approach to storage configuration, opposed to distributed management: operators do not have to configure all storage servers individually to make changes in storage behaviour, but instead make decisions in a logically single location, the controller, with global knowledge of the storage system state.
%
Control plane consists of four components which are described as follows.
First, the \textit{Token Rate Generator} component which communicates with the \emph{QoS (BW) Specification} component in data plane to sync the requested bandwidth specification of each application. Based on these information, it generates a token rate per application. Another control plane component is the \emph{Traffic Shaper} which equally distributes generated tokens into the queue of each corresponding application in the data plane. 
%
Token is a conceptual data structure representing the permission of performing IO requests. Only if a queue holding enough tokens, it will be served by storage system. The other control plane component, the \textit{Virtual Token Buckets}, learns the token rate from the token rate generator and generates corresponding tokens per application. A bucket (buffer) is used per application to keep its corresponding tokens. Note that, the number of generated tokens per application is different. Last, the \textit{Policy Enforcer} is used to deliver policies to meet the QoS requirements. For example, a  policy can be \texttt{<app-1, rate=100 MB/s>} which means application1 can be forced to have a bandwidth of 100 MB/s, no matter how much bandwidth was requested by that application. Actually, the policy enforcer provides a huge flexibility to configure the entire system. It will apply the configuration policies to hundreds of storage servers.

\paragraph{Communication interface}
As shown in Fig.~\ref{fig1}, two communication interfaces are used for this study. One located between the application layer and the control layer, and the other one placed among the control layer and the storage layer. The communication interfaces enable a direct interaction among the layers. For instance, the communication interface located among the application layer and the control layer, permits the control layer to collect the entire applications I/O requirements. However, the other communication interface enables a direct interaction among the control plane and the date planes. Because of this, the data planes can be programmed by the control plane upon QoS requirements.

\subsection{Storage layer}
Storage layer comprises storage servers, data plane on each storage, and OST (object server target). Local data plane runs on each storage server for I/O classification and bandwidth shaping for each application. As shown in Fig.~\ref{fig1}, communication interface is used to enable the storage layer directly interact with the control layer and vice versa. 


